CUF: Continuous Upsampling Filters

Neural fields have rapidly been adopted for representing 3D signals, but their application to more classical 2D image-processing has been relatively limited. In this paper, we consider one of the most important operations in image processing: upsampling. In deep learning, learnable upsampling layers have extensively been used for single image super-resolution. We propose to parameterize upsampling kernels as neural fields. This parameterization leads to a compact architecture that obtains a 40-fold reduction in the number of parameters when compared with competing arbitrary-scale super-resolution architectures. When upsampling images of size 256x256 we show that our architecture is 2x-10x more efficient than competing arbitrary-scale super-resolution architectures, and more efficient than sub-pixel convolutions when instantiated to a single-scale model. In the general setting, these gains grow polynomially with the square of the target scale. We validate our method on standard benchmarks showing such efficiency gains can be achieved without sacrifices in super-resolution performance.

==> fig/overview.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=.99\columnwidth]{example-image-golden}
\hfill
\includegraphics[width=.99\columnwidth]{example-image-golden}
\end{center}
\caption{
% 
\textbf{Outline -- }
A figure summarizing the entire algorithm
}
\label{fig:overview}
\end{figure*}

==> fig/periodic_shuffle.tex <==


\endinput

% \begin{figure}[t]
% \begin{center} 
% \includegraphics[width=0.4\linewidth]{fig/periodic_shuffle_v3.pdf} 
% \end{center}
% \caption{\textbf{Periodic Shuffling~\cite{ShiCHTABRW16} operator:} rearranges the input depth dimension periodically into the tensor spatial dimension increasing its spatial resolution. Typical expansion convolution producing the low features with $r^2$ channels produce each channel independently from each other, despite of spatial correlations expected in their final high-resolution form. We incorporate in our upsampler the assumption that neighboring sub-pixels are expected to be highly correlated.
% }
% \label{fig:ps}
% \end{figure}

==> fig/pos_enc.tex <==
\begin{figure}[t!]
\begin{center} 
\includegraphics[width=0.8\linewidth]{fig/pos_enc_calls.png}
\end{center}
\caption{\textbf{Ablation: positional encoding} --
Performance of positional encoding represented as Fourier (sin/cos pairs) and DCT (cosine only) matches, but the cost associate with calls to sinusoidal projections and also the number of parameters on the hyper-network first layer are halved by two. Metrics obtained upsampling images from Urban-100 dataset \cite{Urban100_Huang2015} by increasing scale factors ($2\times$,$3\times$,$4\times$) using a ABPN~\cite{Du_2021_CVPR_abpn} encoder.
\TODO{conver this to a table}
\cv{Can I move this image/table to the pos encoding appendix? it does not look interesting to me}
}
\label{fig:pos_enc}
\end{figure}

==> fig/qualitative_v0.tex <==
\begin{figure*}[t]
\begin{center}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%first image
\begin{subfigure}{.24\linewidth}
\vfill
    \begin{subfigure}[ht]{\linewidth}
        \vfill
        \begin{subfigure}[t]{0.99\linewidth}
        \includegraphics[width=\linewidth]{fig/qual_error/87_gt.png}
        \caption*{GT - Urban100 - \#008}
        \end{subfigure} 
    \end{subfigure}
\end{subfigure}
\begin{subfigure}{.18\linewidth}
\vfill
    \begin{subfigure}[ht]{\linewidth}
        \vfill
        \begin{subfigure}[t]{0.99\linewidth}
        \includegraphics[width=\linewidth]{fig/qual_error/87_liif.png} 
        \end{subfigure}
         \caption*{SwinIR + LIIF $\times$ 4}
    \end{subfigure}
\end{subfigure}
\begin{subfigure}{.18\linewidth}
\vfill    
        \begin{subfigure}[ht]{\linewidth}
        \vfill
        \begin{subfigure}[t]{0.99\linewidth}
        \includegraphics[width=\linewidth]{fig/qual_error/87_lte.png} 
        \end{subfigure}
         \caption*{SwinIR + LTE $\times$ 4}
        \end{subfigure}
\end{subfigure}
\begin{subfigure}{.18\linewidth}
\vfill        
        \begin{subfigure}[ht]{\linewidth}
        \vfill
        \begin{subfigure}[t]{0.99\linewidth}
        \includegraphics[width=\linewidth]{fig/qual_error/87_cuf.png} 
        \end{subfigure}
         \caption*{SwinIR + CUF $\times$ 4}
    \end{subfigure}
\end{subfigure}
\begin{subfigure}{.18\linewidth}
\vfill    
        \begin{subfigure}[ht]{\linewidth}
        \vfill
        \begin{subfigure}[t]{0.99\linewidth}
        \includegraphics[width=\linewidth]{fig/qual_error/87_gt_crop.png} 
        \end{subfigure}
         \caption*{GT}
    \end{subfigure}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%second image
\begin{subfigure}{.24\linewidth}
\vfill
    \begin{subfigure}[ht]{\linewidth}
        \vfill
        \begin{subfigure}[t]{0.99\linewidth}
        \includegraphics[width=\linewidth]{fig/qual_error/95_gt.png}
        \caption*{GT - B100 - \#86016}
        \end{subfigure} 
    \end{subfigure}
\end{subfigure}
\begin{subfigure}{.18\linewidth}
\vfill
    \begin{subfigure}[ht]{\linewidth}
        \vfill
        \begin{subfigure}[t]{0.99\linewidth}
        \includegraphics[width=\linewidth]{fig/qual_error/95_liif.png} 
        \end{subfigure}
         \caption*{EDSR-baseline  + LIIF $\times$ 3}
    \end{subfigure}
\end{subfigure}
\begin{subfigure}{.18\linewidth}
\vfill    
        \begin{subfigure}[ht]{\linewidth}
        \vfill
        \begin{subfigure}[t]{0.99\linewidth}
        \includegraphics[width=\linewidth]{fig/qual_error/95_lte.png} 
        \end{subfigure}
         \caption*{EDSR-baseline  + LTE $\times$ 3}
        \end{subfigure}
\end{subfigure}
\begin{subfigure}{.18\linewidth}
\vfill        
        \begin{subfigure}[ht]{\linewidth}
        \vfill
        \begin{subfigure}[t]{0.99\linewidth}
        \includegraphics[width=\linewidth]{fig/qual_error/95_cuf.png} 
        \end{subfigure}
         \caption*{EDSR-baseline + CUF $\times$ 3}
    \end{subfigure}
\end{subfigure}
\begin{subfigure}{.18\linewidth}
\vfill    
        \begin{subfigure}[ht]{\linewidth}
        \vfill
        \begin{subfigure}[t]{0.99\linewidth}
        \includegraphics[width=\linewidth]{fig/qual_error/95_gt_crop.png} 
        \end{subfigure}
         \caption*{GT}
    \end{subfigure}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% third image
\begin{subfigure}{.24\linewidth}
\vfill
    \begin{subfigure}[ht]{\linewidth}
        \vfill
        \begin{subfigure}[t]{0.99\linewidth}
        \includegraphics[width=\linewidth]{fig/qual_error/853_gt.png}
        \caption*{GT - DIV2k - \#853}
        \end{subfigure} 
    \end{subfigure}
\end{subfigure}
\begin{subfigure}{.18\linewidth}
\vfill
    \begin{subfigure}[ht]{\linewidth}
        \vfill
        \begin{subfigure}[t]{0.99\linewidth}
        \includegraphics[width=\linewidth]{fig/qual_error/853_liif.png} 
        \end{subfigure}
         \caption*{RDN  + LIIF $\times$ 8}
    \end{subfigure}
\end{subfigure}
\begin{subfigure}{.18\linewidth}
\vfill    
        \begin{subfigure}[ht]{\linewidth}
        \vfill
        \begin{subfigure}[t]{0.99\linewidth}
        \includegraphics[width=\linewidth]{fig/qual_error/853_lte.png} 
        \end{subfigure}
         \caption*{RDN  + LTE $\times$ 8}
        \end{subfigure}
\end{subfigure}
\begin{subfigure}{.18\linewidth}
\vfill        
        \begin{subfigure}[ht]{\linewidth}
        \vfill
        \begin{subfigure}[t]{0.99\linewidth}
        \includegraphics[width=\linewidth]{fig/qual_error/853_cuf.png} 
        \end{subfigure}
         \caption*{RDN + CUF $\times$ 8}
    \end{subfigure}
\end{subfigure}
\begin{subfigure}{.18\linewidth}
\vfill    
        \begin{subfigure}[ht]{\linewidth}
        \vfill
        \begin{subfigure}[t]{0.99\linewidth}
        \includegraphics[width=\linewidth]{fig/qual_error/853_gt_crop.png} 
        \end{subfigure}
         \caption*{GT}
    \end{subfigure}
\end{subfigure}

\end{center}
\caption{
\textbf{Qualitative evaluation} --  CUF combined with different encoders and upsampling scales.
% 
}
\label{fig:qualitative}
\end{figure*}





==> sec/1_introduction_OLD.tex <==
\section{Introduction}
\label{sec:intro}

% --- basic def and applications
Neural-fields represent signals with coordinate-based neural-networks.
They have found application in a multitude of areas including 3D reconstruction\cite{mildenhall2020nerf}, novel-view synthesis~\cite{tancik2020fourfeat}, and many others~\cite{survey_xie2021neuralfields}.
% 
% --- neural fields for point cloud convs
\at{Most importantly, they have also been employed in the realization of convolutional architectures for point cloud data, where grid convolutions (e.g. conv2d, conv3d) are replaced with continuous formulations of convolution kernels~\cite{Hermosilla_2018, WuQL19_PointConv, Boulch2020_ConvPoint}.}

% for large scale point cloud processing in which a continuous formulation of convolutions kernels replaces traditional.
% These continuous convolutions make possible the use of architectures similar to conventional discrete CNNs, but that operate on non-grid structured signals.

\input{fig/teaser} 

In the context of \textit{single image super-resolution} (SISR), some recent approaches make use of coordinate-based formulations  \cite{LIIF_chen2021,lte-lee2022}. 
Their models are based on adding a stack of fully connected layers (four or five) on top of the latent representation produced by deep encoders (convolutional-based~\cite{dong2014learning,EDSR_Lim_2017,RDN_zhang2020} or attentional-based~\cite{ZhangRCAN2018,DaiSOCA2019,SWINIR_liang2021}) that were previously designed for SISR's. 
The deep encoder operates on the same spatial resolution as the input image, 
while the new layers expand it by sampling the encoder's output on a grid over the target resolution. 
The introduction of such a grid supports the coordinate-based formulation, but the extra layers operating at target resolution introduce a considerable overhead, ultimately prohibiting their adoption in low resource settings. 
The best use of the extra resources is also questionable as they do not show a significant increase in performance when compared to \emph{ad hoc} non-continuous up-sampler layers, based on sub-pixel convolutions \cite{ShiCHTABRW16} (\autoref{fig:teaser}). 
In practice, the competitive results, simplicity, and lower demand for resources of sub-pixel convolutions \cite{ShiCHTABRW16} prevents the large adoption of previous continuous formulation by SISR systems.


This paper address the following question: \textit{``can a continuous upsampler based on a neural-fields formulation be created with the same computational budget as its discrete ad hoc counterpart based on sub-pixel convolutions?''}
Our model is inspired by the assumption that the set of discrete upsampling heads supporting different scale factors are highly correlated, 
and so are their up-sampling filters targeting neighboring subpixel positions. 
In principle, given such redundancies it is expected that there might be a low rank shared operation that performs similarly than its discrete counterpart.
Under such an assumption, we review the sub-pixel convolutions operation ~\cite{ShiCHTABRW16} into an operation adopting \emph{Continuous Upsampling Filters} (CUF) that enforces a
shared continuous representation and neighboring relationships in the filter space.

% shared representation and encourages correlations among upsampling filters in the continuous space.
 
\paragraph{Contributions}
\begin{itemize}
\item we investigate the use of neural-fields as a parameterization of \textit{upsampling} layers in \todo{arbitrary scale} super-resolution architectures;
\item the continuity of neural-fields leads to training of naturally compact neural networks (similar PSNR with XX vs. XX parameters), where redundancy is removed by inductive bias, rather than classical distillation.
\item we show how this continuous representation can be instantiated into a discrete one, leading to an efficient inference pipeline (XX flops vs. XX flops);
\end{itemize}

\endinput

% \paragraph{Contributions}
% \begin{itemize}[leftmargin=*]
% \setlength\itemsep{-.3em}

% \item we review the sub-pixel convolution layer 
% and propose a continuous representation of its upsampling filters. 
% By modeling the convolution weights as a neural-fields, in which each dimension of its weights is represented as continuous parameter (target sub-pixel, kernel indexes corresponding to input neighbors and target up-sampling scale), we enforce the coupling of correlations of neighboring values, ignored on the design of the tensor based formulation. 

% % \item our architecture allows a hybrid formulation that at training time supports the instantiation of a discrete sub-pixel based architecture for integer up-sampling factors, while at training time the continuous representation enforces expected correlations.
% \item we propose a hyper-network that can be instantiated into a discrete upsampler and eliminate the hyper-network at inference time for integer upsampling factors, while at training time the continuous representation enforces expected correlations. This is possible, as the neural-field representation of the convolution weights is independent of the image content and can be precomputed given an integer upsampling factors, thus, in those cases our hybrid formulation can be instantiated into a sub-pixel convolution formulation at test time.

% \item In the arbitrary-scale use-case, the architecture of our upsampling head further assumes that the expansion of the spatial coordinates and the projection projection of feature channels can be decoupled. As a results, its design combines depth-wise and point-wise convolutions into an upsampler considerably lighter than previous arbitrary scale upsamplers (\autoref{tab:params}).

% \item We propose the use of DCT based positional encoding for projecting the parameters that define the convolution weights dimensions, as a smaller kernel basis to aid preventing spectral bias. 
% %we show that kernel projection can be made at smaller basis set (half the size of sin/cos based models) and significantly smaller than random basis set. 

% \item A practical contribution of our work is to be the first time and arbitrary scale upsampler is efficient enough to be applies at lightweight and extremely light-weight models.

% \item Quantitative and qualitative results show that our model matches or outperform previous method while demanding significantly less computational resources.

% \end{itemize}


==> sec/2_related_OLD.tex <==
\section{Related work}
\label{sec:related}

% Super resolution is an area of active research that has substantially benefited from deep neural networks. A large number of encoders has been developed in the last decade exploring different components such as, but not limited to, convolutional layers \cite{dong2014learning,EDSR_Lim_2017,RDN_zhang2020} and attention-based layers \cite{ZhangRCAN2018,DaiSOCA2019,SWINIR_liang2021}. 
% Our investigation is focused on the upsampler component specifically, and can be combined with different choices of encoders.
% For this reason, this section presents a  literature review  focused on differentiating up-sampling layers. A number of other SISR research topics can be found in the following surveys \cite{surveyWang2021,surveyAnwar2020,surveyBashir2021}. 
% As our model has a neural-fields based formulation, we also point the reader to the survey in this topic in \cite{survey_xie2021neuralfields}.

\paragraph{Single scale}
Different frameworks based on deep architectures vary in the formulation and location of the upsampling operator. 
% 
\begin{itemize}
\item in the \textbf{pre-upsampling framework}\cite{dong2014learning}, the super resolution problem is stated as the task of recovering a high quality super-res image starting from an initial approximation obtained using a non-trainable upsampler (e.g. bicubic). This enables arbitrary input size and scaling factors, but can introduce side effects such as noise amplification and blurring.
Further, computational complexity is significant, as these model operate directly at the target resolution.
\item in the \textbf{post-upsampling framework}~\cite{ShiCHTABRW16}, a deep encoder is applied that
preserves the spatial resolution throughout, followed by a shallow up-sampling component placed at the end of the model; given their efficiency, most mainstream approaches adopt \emph{Post-upsampling}~\cite{SRCNN_Dong2016, ESRGAN_Wang2018, EDSR_Lim_2017, RDN_zhang2020, ZhangRCAN2018, SWINIR_liang2021}.
\end{itemize}
% Lim et al. \cite{EDSR_Lim_2017} expanded this to multiple scales, introducing the idea of sharing the encoder with shallow, per-scale upsampling heads.
% \AT{removed as this is a multi-scale one?}


% , ranging
% from very deep encoders \cite{SWINIR_liang2021} down to 
% architectures targeting low resources devices (such as  \cite{Du_2021_CVPR_abpn}.
% It is adopted by a diverse set of models ranging from very deep architectures inspired on models holding SOTA results on  classification and detection 
% (such as 
% \cite{SWINIR_liang2021} that is based on 
% Swin Transformer architecture \cite{liu2021Swin}) down to architectures targeting low resources devices (such as  \cite{Du_2021_CVPR_abpn}). 
%
We investigate the impact of an implicit upsampler in the \emph{Post-upsampling Framework} covering  a diverse set of architectures ranging from larger \cite{liu2021Swin} to extremely lightweight models \cite{Du_2021_CVPR_abpn}. 
% The impact of our implicit upsampler on other frameworks, such as those with hidden features at multiple resolutions \cite{Hu_2019_CVPR_Workshops}, that consequently adopt multiple upsampling layers, is left as future work.

\paragraph{Multi-scale} 
Hu et al. \cite{metasr_hu2019} were the first to introduce an upsampler that supports multiple scales and non-integer scale factors. 
In their meta-learning based approach, named MetaSR, a hyper-network is conditioned on 
the target scale factor and 
on the output pixel relative coordinates (ie. the difference between HR and LR grids covering the same normalized global space). 
Their complete model consists of (1) transforming the input image using an encoder into LR deep features; 
(2) upsampling the deep features into the HR target space (using nearest-neighbors);
(3) using the hyper-network to produce a filter set per target relative position and scale; (4)  processing the enlarged HR feature map into the final output using the corresponding weights. 
In \cite{LIIF_chen2021}, Chen et al. introduce the LIIF upsampler that 
eliminates the use of a hyper-network (step 3) by 
extending the sampled HR  features (step 2) with extra channels representing the relative coordinates and target scale.
Their combined features are further processed through a stack of 5 dense layers 
inspired by the multi-layer perceptron (MLP) architecture typically adopted as the end-to-end model in neural-fields formulations. 
Recently, Lee and Jim \cite{lte-lee2022} propose the LTE upsampler that further enhance the features fed as input to the MLP layers.
In their model, the output of the encoder is processed by three extra trainable layers 
associated with the amplitude, frequency and phase of sin/cosine waves.
The resulting projection in HR is used as the input to the stack of $4$ MLP layers.
In order to further improve the results they also adopt a global skip connection with a bilinear up-scaled version of the input around the full model, such that the deep model focus on the computation of the residual between to the closed form approximation and the final result. 
In practice, LIIF and LTE may also increase the number of feature channels in the HR space as their MLP layers have more neurons ($256$) than the number of channels produced as the  encoder output ($64$ for  encoders such as EDSR\cite{EDSR_Lim_2017} and RDN\cite{RDN_zhang2020}).

The design of our implicit upsampler contrasts with the previous work by (i) adopting a neural-fields formulation that 
focuses the sensitivity of our hyper-network to small changes in the representation of scale and relative position (reducing the spectral bias); (2) moving the computational burden into the implicit upsampler, while reducing the operations performed in the HR space at the same time, preserving the number of channels produced by the deep encoder. 

% (not adopted in MetaSR), 
% but of the upsampler transformation only (and not of the concatenation of the feature map, position and scale representations as in LIIF and LTE).
% Our proposed architecture moves the computational burden into the implicit upsampler computation, while reducing the operations performed at the HR space and also by preserving the number of channels as those produced by the deep encoder.

We further show that in the most typical application case, of up-sampling an image by an integer scale factor, our implicit upsampler produces an upsampler with a similar or fewer number of operations than the original single scale sub-pixel convolution, producing results with equal or superior quality.

A number of other SISR research topics can be found in the following surveys \cite{surveyWang2021,surveyAnwar2020,surveyBashir2021}. 
As our model has a neural-fields based formulation, we also point the reader to the survey in this topic in \cite{survey_xie2021neuralfields}.

\input{fig/architectures}
\vfill
\endinput

% In LIIF, the stack of dense layers is responsible for mapping from the HR feature space up to the output RGB-channels.
%Note that while in the MetaSR each element of the HR feature map is further processed by a single layer, in LIIF they are processed by all the extra layers introduced by the addition of the MLP layers.



% \paragraph{Spectral Bias}
% \CV{Should we do a brief review of Spectral bias as pos encoding literature here?} 

% \paragraph{Hyper-networks} 
% \CV{Should we do a brief review of hyper nets literature here?} 

==> sec/3_method_OLD.tex <==
\section{Method}

A deconvolution layer \cite{ZeilerTF11}, also known as backwards convolution, is a well known upsampling operator adopted in several deep architectures. Among its properties, it has already been shown that bicubic interpolation is a special case of  deconvolution layer \cite{Long2015cvpr,Dong2016TPAMI}. 
A fundamental limitation of deconvoluton is that it operates on the output HR feature map. To alleviate this problem, Shi et al.~\cite{ShiCHTABRW16} proposed an efficient alternative that operates on the input LR feature map, named the sub-pixel convolution layer. We start with a discussion of sub-pixel convolution and its limitations and propose a new type of continuous upsampler that targets those limitations.


\subsection{Periodic Shuffling}
\label{sub:subpixel}
% 
The sub-pixel convolution layer combines an expansion convolution with a \emph{periodic shuffling} ($\mathcal{PS}$) operator --  also known as \emph{depth to space} or \emph{pixel-shuffle} operator.
\AT{r is undefined}
More specifically, first a convolution with a kernel $\mathbf{W}$ of size $k \times k$ expands the feature space from $n_{in}$ input feature channels into $r^2 n_{out}$ output feature channels, i.e. $\mathbf{I}'_{out} = \mathbf{W} \ast \mathbf{I}_{in}$, ignoring the bias term for simplicity. The result is a tensor of size $h \times w \times r^2 n_{out}$ for an input feature map of size $h \times w \times n_{in}$. This tensor is then rearranged into a feature map of a larger spatial resolution and $n_{out}$ channels by the $\mathcal{PS}$ operator. 
The $\mathcal{PS}$ operator periodically rearranges the channels with:
% 
% \begin{equation}
% \mathbf{I}_{out}(x, y, c) = \mathcal{PS}[\mathbf{I}'_{out}](x, y, c) = \mathbf{I}'_{out}(\lfloor x / r \rfloor, \lfloor y / r \rfloor, c [r \bmod(y, r) + \bmod(x, r)])
% \end{equation}
% 
\AT{is this math needed? feels like a ref to fig2 should be enough?
Unless the math is reused somewhere else}\KS{In either case we should add more dimension annotation to fig2.}
% 
where $x, y$ are the sub-pixel indices and $c$ is the channel index.


A fundamental limitation of the combined expansion operation of $\mathbf{W}$ and $\mathcal{PS}$ is that correlations among sub-pixels in the $r \times r$ blocks in the output are ignored.
Existing correlations among neighbors may be learned from training data, but are not enforced by the expansion convolution structure \emph{per se}.
As an example, assuming $n_{out} = 1$, the $\mathcal{PS}$ operator gets the value of the first sub-pixel of each $r \times r$ block from the first channel of $\mathbf{I}_{in}$, second sub-pixel from the second channel, and so on \autoref{fig:ps}. 
This means each set of sub-pixels with the same relative positions in the $r \times r$ blocks are generated with  the same kernel (a subset of $W$), that is not reused for generating other set of sub-pixels with different relative positions. 
This thus ignores any prior assumption that close-by target sub-pixels are highly correlated and hence the corresponding kernels should also be correlated. \KS{My reading of this is that channels in a CNN are not necessarily correlated with each other. This can be learned from training data, but is not enforced. Is this correct? If so, I feel like we can say things more succinctly and intuitively here.}

A second limitation of the expansion-convolution $\mathbf{W}$ 
is that it does not support sub-pixels with different indexes than those associated with a given $r$, i.e. it supports a single scaling factor. A direct consequence of this limitation is the need for one upsampling head per target scaling factor.
Adding to that, both $\mathbf{W}$ and $\mathcal{PS}$ assume the same relative positions are replicated across the target image, and do not support non-integer scale factors that create non-periodic grids, as necessary for arbitrary-scale upsampling. 

\subsection{The continuous upsampler}
\label{sub:singlescale}

To overcome the limitations mentioned, we propose a neural field based formulation of the convolutional kernel with continuous parametrization of the relative sub-pixel coordinates and target scale. 
Specifically, we introduce the \emph{continuous upsampling operator}, a continuous function that outputs a convolution kernel for the sub-pixel with a certain relative coordinate:

% \myfunc{\mathbf{S}(\epsilon_x,\epsilon_y)}{\mathbb{R}^2}{\mathbb{R}^{n_{in}\times~k~\times~k~\times~n_{out}}}
\begin{equation}
\mathbf{S}(\epsilon_x,\epsilon_y)~\colon~\mathbb{R}^2\to \mathbb{R}^{n_{in}\times~k~\times~k~\times~n_{out}}
\end{equation}
where $\epsilon_x$ and $\epsilon_y$ are the relative coordinates. 
These kernels are then applied to the input image to get the value of a pixel of the output image with

\begin{equation}
    \mathbf{I}_{out}(x, y) = \left[\mathbf{S}\left(\epsilon_x, \epsilon_y \right) \ast \mathbf{I}_{in}
    \right]
    (
    \lfloor x / r \rfloor, \lfloor y / r \rfloor),
\label{eq:inout}
\end{equation}
where $\epsilon_x = \bmod(x, r) / r$ and $\epsilon_y = \bmod(y, r) / r$. This operation thus first computes the relative sub-pixel position, the corresponding convolution kernel, and finally applies the kernel to the input image to get the corresponding subset of output pixels. The neural network representing the functional $\mathbf{S}$ introduces a coupling of kernels for different relative sub-pixel positions. Furthermore, 
as $S$ is continuous, we can specify any continuous upscaling factor $r$. The operation works for arbitrary sub-pixel coordinates and scaling factors, so long as we trained the network accordingly. That is, \autoref{eq:inout} 
solves the problem of supporting non integer values of $r$.
The multi-scale and arbitrary-scale formulations are further discussed in \autoref{sub:multicale}.

At inference time, when targeting an integer upscaling factor $r$, the hyper-network representing $S$ can be decoupled from the layers processing the input image and queried to pre-compute the weights of an expansion convolution $W$ corresponding to $r$.
In those cases, at inference time our model can be instantiated to be as efficient as a sub-pixel-convolution based architecture, 
while at training time the neural fields formulation sustain the continuous modeling enforcing local correlations within the convolution weights.

\input{fig/periodic_shuffle}


\paragraph{Kernel indices as inputs} 
In order to fully represent the up-sampling convolution as continuous, we further introduce a continuous parametrization of its kernel indexes  $k_i, k_j$. Thus, the hyper-network representing the convolution functional $S$ can be expressed as:
% \begin{equation}
%     \myfunc{\mathbf{S}(\epsilon_x,\epsilon_y, k_i, k_j)} {\mathbb{R}^{4}}{\mathbb{R}^{n_{in} \times n_{out}}}.
% \end{equation}
\begin{equation}
\mathbf{S}(\epsilon_x,\epsilon_y,k_i,k_j)~\colon~\mathbb{R}^4\to \mathbb{R}^{n_{in}\times~n_{out}}
\end{equation}


\subsection{CUF: Continuous Upsampling Filters}
%\subsection{Extensions and Architecture}
\label{sec:architecture}
 This subsection describes the architecture proposed for \emph{CUF}: a hybrid up-sampling head based on the continuous upsampler operator in which a single hyper-network 
 can both be instantiated into a sub-pixel convolution for supporting integer scale upsampling, or used to produce  non-integer upsampling.
 

\input{fig/single_scale_arch}
\paragraph{Continuous depth-wise convolution} Depth-wise convolutions are those in which the convolution operation is applied per input channel~\cite{Chollet17}.
Our CUF upsampler head archtecture is composed of a depth-wise separable convolution, followed by point-wise convolutions \autoref{fig:single_scale_arch}. Our model decouples the task of expanding the spatial dimensions of the feature map produced by the deep encoder from the task of projecting its channels into the target channels (typically RGB).  
In this decoupled formulation, the upsampler adopts an continuous depth-wise convolution with $n=n_{in}=n_{out}$, further simplifying $S$ can to:
\begin{equation}
\mathbf{S}(\epsilon_x,\epsilon_y,k_i,k_j)~\colon~\mathbb{R}^4\to \mathbb{R}^{n}
\end{equation}

A practical consequence of adopting the depth-wise formulation is efficiency. 
When compared to the sub-pixel convolution upsampler, our upsampler head reduces both the number of parameters and FLOPs whenever $k \times k + N_{in} + N_{out} < N_{out}\times k \times k$ as the cost associated with pre-computing the weights for a given integer up-sampling scale can be neglected when compared to the operations performed on the image grid.

% The number of multiplications is also reduced whenever $k*k*r*r + N_{in}*r*r +  N_{out}*r*r < N_{out}*k*k*r*r$
% $W,H*N_IN *N_out*k*k*r*r$
% $W,H,N_IN  *k*k*r*r + 
% W,H,N_IN * N_IN*r*r + 
% W,H,N_IN * N_OUT*r*r$


\paragraph{Representing coordinates and indices} 
\AT{why is this ``better'' than the NeRF sin/cos? unclear.}
\AT{also, connection to previous section is unclear, this popped up quasi-randomly?}
\CV{We are trying to make all things affordable, DCT is a real transform which results in a single real number per data point. In contrast, a DFT results in a complex number (real and > imaginary parts) which requires double the memory for storage.}
\todo{We input the relative sub-pixel coordinates and the kernel indices into $S$, which is susceptible to spectral bias that hampers the MLP from learning fast changes in its inputs~\cite{pmlr-v97-rahaman19a,Tancik2020}. In order to alleviate this, we represent both with positional encoding. Previous works mostly adopt sines and cosine pairs inspired by the Fourier Transform \cite{Rahimi_NIPS2007,tancik2020fourfeat}. 
We instead adopt a cosine only set inspired by the Discrete Cosine Transform basis.  This has the same representation power but simplified representation as all functions encoded are real. More specifically, we adopt the following 2D-basis:

\begin{equation}
 cos\left( \frac{(2x+1)f_i\pi}{2} \right) cos \left( \frac{(2y+1)f_j\pi}{2} \right),
\end{equation}
where $x,y$ are the 2D coordinates of the parameter being encoded (normalized into the interval $[0,1]$), and $f_i, f_j$ are frequencies uniformly sampled from $0$ to $f_\text{max}$. The DCT based formulation allows a semantic interpretation of its hyper-parameters, so that  $f_\text{max}$ is upper bounded by  the maximum wavelength seen during training for the input parameter being encoded (following Nyquist limit).}


\subsection{Multiple-scale and Arbitrary-scale models}
\label{sub:multicale}
A common practice in multi-scale settings, where models commonly support
a set of integer up-scaling factors, 
is to share a deep feature extractor across scales, while one of (or a stack of) expanding convolutions are trained per scale due to the dependency of the sub-pixel convolution upsampler on the scaling factor $r$.
In our neural-fields based formulation, it is possible to condition $S$ on scale such that the hyper-network receives $r_w, r_h$ as extra inputs. Similar to the relative coordinates and kernel indices, we apply positional encoding on these factors.
The same hyper-network can then be shared during training, and used to produce the weights of a PS-based architecture as pre-processing at inference time. In this scenario, where the upsampling factor is an integer scale, the computational cost of producing the convolution weights is independent of the image size but instead is proportional to $k\times~k~\times~r_w~\times~r_h$.

An extra advantage of conditioning on scale is to support arbitrary-scale upsampling factors where $r_w, r_h$ can assume any continuous value. 
In this case, the periodicity observed for integer scale factors can not be assured.  Similar to previous work \cite{metasr_hu2019, LIIF_chen2021,lte-lee2022}, the expansion is obtained by producing a grid over the target output, that is mapped into the relative coordinates ($\epsilon_x, \epsilon_y$), and also used to sample the LR feature map and suppress the need of a later $PS$. 

% Similar to previous arbitrary-scale methods, the feature corresponding each position in the grid is obtained using nearest-neighbor (NN).
% In order to support $k~\times~k$ filters, over the LR feature map, the corresponding neighborhood is folded into channels prior to the NN sampling.

\autoref{fig:arbitrary_scale_arch} and \autoref{tab:archtectures} presents our arbitrary scale upsampler architecture and its comparison to previous works. We make the main network shallower ($1$ depth-wise continuous convolution and $2$ dense layers) in order to reduce the number of layers that operate at the target spatial resolution.
At the same time, our upsampler head is considerably lighter than previous arbitrary scale methods, not only by the use of a depth-wise convolution
but also by keeping the same number of channels produced by the features encoder in the main network ($64$ versus $256$ in LIIF and LTE).
When performing integer scale up-sampling at inference time, the hyper network cost can be neglected and upsampler head instantiated into a PS-based head (\autoref{fig:ps}). When performing non-integer upsampling, the costs with processing the hyper-network layers is proportional to the target image resolution, but still smaller than a single dense layer of LIFF and LTE heads, due to the adoption of reduced number of channels (one dense layer over $64$ features is $16\times$ smaller than its version using $256$ neurons).  

% The deptwise convolution is performed
% % Dense 580 → 256, ReLU
% The hidden dense layers of main network reduces its processing by a factor of 16. The final layer by a factor of 4. When applied to integer scale factor the cost of producing the Deptwise-Convolution weight matrix of size the $r*r*k*k*N_{in}$ is very small compared to the operations that are dependent on the image, and can be 
% ignored.
% For arbitrary 


% The number of channels in the main network is kept as the same as produced by the deep encoder (64 in the case illustrated) while previous 

\endinput 

% where by indexing pixels by $x, y$ and channels by $c$:
% 
\begin{equation}
\lfloor x / \scale \rfloor, \lfloor y / \scale \rfloor, c [\scale \bmod(y, \scale) + \bmod(x, \scale)]
\end{equation}

==> sec/4_results_OLD.tex <==
% \input{tab/hyper_params}
\input{tab/params}
\section{Results}
\subsection{Experimental setup}
% 

\paragraph{Encoders}
We apply CUPs to a variety of \textit{encoders}, to both show its generality, as well as its performance gains in a variety of settings:
% 
\begin{itemize}
\item state-of-the-art model for super-res such as the SwinIR encoder  \cite{SWINIR_liang2021} based on Swin-transformers \cite{liu2021Swin}.
\item convolutional-based models such as EDSR-baseline~\cite{EDSR_Lim_2017} and Residual Dense Networks (RDN)~\cite{RDN_zhang2020}; 
\item architectures for lightweight and extremely lightweight inferences, respectively SwinT-lightweight~\cite{SWINIR_liang2021} and ABPN~\cite{Du_2021_CVPR_abpn}.
\end{itemize}
% 
Table \ref{tab:params} contrasts the ablated encoders' composition and size,  Hyperparameter settings can be found in the supplementary material.



% \paragraph{Training Hyper-params} 
% \autoref{tab:hyper} contains the hyper-parameters adopted for training the ablated models, taken from their original single-scale training settings. All models are trained for 1k epochs with  $\mathcal{L}_1$ loss and ADAM optimizer by setting $\beta_1=0.9$,
% $\beta_2=0.999$,
% and $\epsilon=1e^{-8}$. We use a step-wise learning rate schedule that is halved at epochs $[500,800,900,950]$. Unless mentioned, models were trained with random scales by sampling the scale factor uniformly within the continuous interval  
% $[1, 4]$.
% In order to ensure that the dimensions within the training mini-batch match despite heterogeneous scale factors, we first scale each image as required and then apply the same crop size to each image.
% \todo{In order to enforce matching dimensions within the training mini-batch containing LR-HR pairs at different up-sampling scales, both LR and HR crops were taken at same fixed size (\autoref{tab:hyper} no matter the scale factor.}
% \AT{don't understand}
% The matching dimensions is enforced by randomly selecting a window with the chosen fixed size over the HR ground truth. 

% \AT{was there a main codebase? we'd state as much if so? or mostly snippets here and there. Further, if you say that, it's tricky, as the licences need to be correct...? danger noodle}
% \todo{Our code is built on top of previous work codebases} (\cite{EDSR_Lim_2017,LIIF_chen2021,lte-lee2022,SWINIR_liang2021,Du_2021_CVPR_abpn}) and will be public upon acceptance. We thank their authors for sharing their codes.

\paragraph{Datasets}
All models are trained using from the DIV2K dataset training subset ($800k$ images), introduced at the~NTIRE~2017 Super Resolution Challenge~\cite{DIV2k_Timofte2017}.
Similarly to previous works, each image is randomly cropped 20 times per epoch and augmented with random flips, and 90 degrees rotations. 
We report peak signal-to-noise ratio (PSNR) results on the DIV2K validation set (100 images)\footnote{\at{Note the models we compare to also do not report results on the test-set, which is not publicly available.}}, on \emph{RGB} space.
We test our models on additional well known SISR datasets (Set5 \cite{SET5_Bevilacqua2012} -- 5 images;  
Set14 \cite{Set14_Zeyde2010} -- 14  images; 
B100 \cite{B100_Martin2001}  -- 100 images;
and Urban100 \cite{Urban100_Huang2015} -- 100 images), in which, following previous works, PSNR is measured in the luminance channel of the \emph{YCbCr} space.


\input{tab/benchmarks}
\input{tab/sota}


\subsection{State-of-the-art comparisons}
\lorem{1}

\subsection{Effect of positional encodings}
\label{sec:posenc_results}
\lorem{1}

\Table{sota} and \Table{benchmarks} show the quantitative comparison between our implicit upsampler, sub-pixel convolution upsampler heads and previous methods for arbitrary-scale up-sampling combined with different encoders.
\Table{sota} contains 
in-domain results: models trained and tested on DIV2k dataset splits. \Table{benchmarks} presents out-of-domain results: models are trained on DIV2k, but tested on a set of different datasets.
\todo{The upsampling ratios larger than $4$ are seen during test time only.}
\AT{why is it important to show their performance then? Can't we just show x6 and call it a day? what value added are 18, 24, 30? This would make Table 4 MUCH easier to read too.}
The models adopting sub-pixel convolution are fixed-scale models, that is, one model is trained per target scale
and they do not generalize to unseen nor fractional scales. On the remainining rows,  presenting arbritary-scale upsamplers (MetaSR~\cite{metasr_hu2019}, LIIF~\cite{LIIF_chen2021}, LTE~\cite{lte-lee2022}), a single model is trained and tested across different upsampling ratios.

The tables also contain results obtained by the use of Geometric Self-ensemble \cite{EDSR_Lim_2017}, commonly adopted in SISR,  where the results of rotated versions of the input image are averaged at test time.  Note that LIIF and LTE results adopt Local Self-ensemble ($lc$), where the result of applying the upsampler at $4$ shifted grid points is averaged. The adoption of local self-attention induces an overhead during both training and testing time. It may also introduce confounding factors to the optimization process that invalidate direct comparison to the fixed-scale upsampler\footnote{During back-propagation the encoder gradients are averaged.}.

Our method is the first to match or surpass fixed-scale performance across all encoders in both single-pass inference and self-ensemble scenarios. Previous arbitrary-scale methods surpass the fixed scale results when added on top of the smaller encoder (EDSR $~1.5\mathrm{m}$ parameters) but do not present similar gain when combined with larger models. 
We conjecture that the extra capacity introduced by those upsamplers ($300\mathrm{m}-500\mathrm{m}$ parameters - See \autoref{tab:params}) has a larger impact on  the performance of small encoders than on the largest ones, where the fixed scale training, based on sub-pixel convolution still dominated the best results prior to our proposal. 

Our upsampler, on the other hand, does not introduce an increase in capacity. On the contrary, its total number of parameters 
is smaller than those of the compositions adopting sub-pixel convolution on the baseline models investigated. 
Despite of the reduced capacity, our model surpasses the fixed scale baselines adopting  sub-pixel convolutions for the different encoders tested at the same time that  matches or surpass the previous arbitrary models that proposed models considerably more heavy computationally. 

Qualitative comparisons covering the different encoders and compositions are presented in \autoref{sup:qualitative}.

% and \Table{ablations}
% \Table{lightweight}. 





% \paragraph{Disentangling the impact of self-ensemble on training.} self-ensemble  consists of....
% Traditionally models apply self-ensemble as a post processing of trained models. In \cite{LIIF_chen2021,lte-lee2022} self ensemble is adopted during training... Thus, the error of forward passing 4 nearest points are backpropagated throught the full network.
% In our ablations we disentangle the impact of adopting self-ensemble as a post-processing versus during training approach.

% For increasing their final performance, during inference time both EDSR and RDN ensemble copies of the input image transformed by that have their response average into a single output.
 
 





\subsection{Lightweight and extremely lightweight models}

\input{fig/abpn}

\input{tab/lightweight}



\subsection{On the use of positional encoding}
% \input{tab/posenc}
\input{fig/pos_enc}






% \subsection{Weights Visualization}
% \input{fig/filters}



==> sec/X_instructions.tex <==
% --- repeat the title (AT: haven't found a more elegant way to do this...)
\twocolumn[
\centering
\Large
\textbf{\LaTeX\ Author Guidelines for \confName~Proceedings (2022)}
\vspace{1.0em}
] %< twocolumn
\appendix

\setcounter{section}{0}
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of cvpr.sty to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the CVPR70 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


% Update the cvpr.cls to do the following automatically.
% For this citation style, keep multiple citations in numerical (not
% chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
% \cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
